HopGNN: Boosting Distributed GNN Training Efficiency via Feature-Centric Model Migration

Distributed training of graph neural networks (GNNs) has become a crucial technique for processing large graphs. Prevalent GNN frameworks are model-centric, necessitating the transfer of massive graph vertex features to GNN models, which leads to a significant communication bottleneck. Recognizing that the model size is often significantly smaller than the feature size, we propose LeapGNN, a feature-centric framework that reverses this paradigm by bringing GNN models to vertex features. To make it truly effective, we first propose a micrograph-based training strategy that trains the model using a refined structure with superior locality to reduce remote feature retrieval. Then, we devise a feature pre-gathering approach that merges multiple fetch operations into a single one to eliminate redundant feature transmissions. Finally, we employ a micrograph-based merging method that adjusts the number of micrographs for each worker to minimize kernel switches and synchronization overhead. Our experimental results demonstrate that LeapGNN achieves a performance speedup of up to 4.2x compared to the state-of-the-art method, namely P3.

==> tex/design0.tex <==
\section{Design of \pname{}}

In this section, we describe the key idea of \pname{}
that addresses the aforementioned challenges.
Then, we introduce two optimizations to further improve
the performance of \pname{}.

\subsection{Data Locality in Micrographs}
\label{design0}


\textbf{Micrographs:} For each vertex in a mini-batch,
we need to create a micrograph using k-hop sampling
during GNN training. For the convenience of discussion,
we use the vertex ID to denote its corresponding
micrograph in the paper. A subgraph may consist of 
multiple micrographs. Figure~\ref{fig:subgraph_bs2}
shows an example of micrographs. The subgraphs in the figure
are sampled from the graph in Figure~\ref{fig:graph}.
In the example, we assume that (1) the size of a mini-batch
is two, (2) vertex feature data and graph topology data
are distributed across two GPU servers, and (3)
the fanout is 2 and number of computation layers is 2.
The subgraph corresponding to the mini-batch [6, 3]
consists of micrograph 6 and micrograph 3.
The subgraph corresponding to the mini-batch [5, 0]
consists of micrograph 5 and micrograph 0.

For improving data locality and reduce communication cost, 
it is very likely that the root vertex of 
a micrograph is stored in the same partition as its 
fanout neighbors. Therefore, the vertex features of
the fanout neighbors tend to be distributed on the server
where the feature data of its root vertex is located.
We continue to use the example for illustration.
In Figure~\ref{fig:graph}, we use different 
colors to represent the home locations of vertices (e.g.,
yellow denotes server 0 and blue denotes server 1).
In the example in Figure~\ref{fig:subgraph_bs2}, we need to 
retrieve the subgraph for the mini-batch [6, 3]. 
As a result, for subgraph 0, 6 and 3 become the 
root vertices of micrograph 6 and micrograph 3 respectively. 
Because of data locality, in micrograph 6, vertices 6, 5, and 7 
are retrieved from server 0. When training using 
micrograph 6, 3 feature 
vectors (for vertices 6, 5, and 7) are read from server 0.
%  and 1 feature vector (i.e., vertex 1) are from server 1. 
% \frac{3}{4} 
They account for $3/4$=75\% of the total amount of the feature vectors 
required for training micrograph 6. Similarly, when training 
micrograph 3, 3 feature embedding vectors are read from server 1. 
They account for $3/5$=60\% of the total amount of the feature  
vectors required for training micrograph 3. 
The feature data locality also exists in subgraph 1.

\begin{figure}
        \centering
        \subfigure[]{
                \includegraphics[height=2.1in]{subgraph_bs2.pdf}
                \label{fig:subgraph_bs2}
        }
        \subfigure[]{
                \includegraphics[height=2.1in]{micrograph.pdf}
                \label{fig:micrograph}
        }
        \caption{(a) Two subgraphs for mini-batch [6,3] and [5,0] respectively. 
(b) Partition the subgraphs to micrographs, each of which is
trained on a GPU server.}
\end{figure}

To demonstrate the generality of this observation, we conduct 
experiments on three real-world open-source graph datasets 
(representing small, medium, and large-scale datasets) with 
various number of model layers and distributed machines. The 
first two datasets are partitioned with METIS~\cite{metis98} 
used in DGL~\cite{dgl-arxiv19}, and the last large dataset is partitioned with 
a heuristic algorithm for GNN~\cite{pagraph-socc20} because 
the METIS algorithm runs out of memory when partitioning
the graph.

We collect the number ($N_{co-located}$) of non-root vertices 
which are co-located with its root vertex in a micrograph 
during GNN training. Then, we compute the ratio ($ratio_{locality}$) 
of $N_{co-located}$ and $N_{total}$, where $N_{total}$ is the 
total number of vertices in a subgraph. We show $ratio_{locality}$ 
in Figure~\ref{fig:same_ratio}. The horizontal red line represents the 
ratio ($ratio_{random}$) under a random distribution without locality, 
while the height of the bars represents the value of $ratio_{locality}$. 
We observe that $ratio_{locality}$ is consistently larger than 
$ratio_{random}$. Furthermore, as the number of GPU servers is 
increased from 2 to 16, the difference between $ratio_{locality}$ 
and $ratio_{random}$ increases from 1.59$\times$ to 10.60$\times$.

We attribute this observation to the advanced graph partitioning 
algorithms used in GNNs such as METIS~\cite{metis98} and 
GNN-specific heuristic algorithms~\cite{pagraph-socc20, bgl-nsdi23, bytegnn-vldb22}. 
These algorithms aim to minimize feature transmission across machines 
by assigning neighboring vertices to the same graph partition for
higher data locality. Therefore, when sampling k-hop neighbors from 
a root vertex, a large number of vertices in the same micrograph
are co-located with the root vertex on the same GPU server.

\begin{figure}
	\centering
	\includegraphics[width=3.2in]{same_ratio.pdf}
	\caption{The ratio values with various number of layers and machines. The x-axis represents the "number of model layers - number of machines".}
	\label{fig:same_ratio}
\end{figure}



==> tex/design3-old.tex <==
\subsection{\techC{}}
\label{design3}


%\begin{figure}
%	\centering
%	\includegraphics[width=1.6in]{et_N.pdf}
%	\caption{The initial TT of one interation training with N machines.}
%	\label{fig:et_N}
%\end{figure}
%
%\begin{figure}
%	\centering
%	\includegraphics[width=1.6in]{et_random_remove.pdf}
%	\caption{Random remove for GNN training with three distributed machines.}
%	\label{fig:et_random_remove}
%\end{figure}

While sending micrographs to the machine where the root vertex feature resides can maximize the reduction of remote vertex feature transmission, this approach may not always be the most optimal solution for overall training performance, especially in scenarios with a large distributed scale. This is because it leads to the generation of many micrographs, resulting in time overhead in frequent launching of GPU kernels and synchronization time at the end of each time step. In our experimental results, when training the GCN model across four machines on the ogbn-arxiv dataset with batch size 2048, in default method, the average training time of one epoch is 7.59s, whereas after only using \techa{} it becomes 8.37s.


\begin{figure}
	\centering
	\subfigure[The initial TT.]{
		\includegraphics[width=1.3in]{et_N.pdf}
		\label{fig:et_N}
	}
	\subfigure[Random remove of TT.]{
		\includegraphics[width=1.7in]{et_random_remove.pdf}
		\label{fig:et_random_remove}
	}
	\caption{Example of model migration trace and removal.}
	\label{fig:default-design1}
\end{figure}


We introduce a Trace Table (TT) to better illustrate the main idea of our solution and the details.
Figure~\ref{fig:et_N} shows an initial TT for one iteration of first epoch training.
The row identity represents the ID of each model replica. Each column represents a time step where each model completes training a micrograph. We use different colored squares to represent different machines, and machine IDs are labeled inside the squares.
The TT shows which machine each model is executed on for each time step after using \techa{}.  For example, during the time step 0, model $i$ trains the micrograph on machine $i$.  Then, model 0 sequentially migrates to machine 1, machine 2, and so on, until it reaches machine N-1 to finish all micrographs training. The other models follow a similar pattern at the same time.
Since a subgraph is divided at most into N micrographs, there are a total of N time steps in the initial TT. 

To overcome the problem of increasing overall training time, the main idea is to reduce the number of divided micrographs, so that the times of GPU kernel launching and synchronization becomes less. For each model, removing a micrograph means removing a time step from the initial TT. However, the specific solution is not straightforward because there are three questions need to be addressed.
\begin{enumerate}
\item How many micrographs should be removed for each model? If the left value is too small, the number of remote feature transmission will become large. The most extreme case is that one subgraph equals one micrograph which results in a significant amount of feature communication. If the left value is too large, frequent launching of GPU kernels and synchronization can not be reduced.
\item Which micrographs should be removed for each model?  
Random removal may cause multiple models to train micrographs on a single machine at the same time step. For example, Figure~\ref{fig:et_random_remove} represents the initial TT of 3 machines before removing the micrographs and the TT after each model randomly removes a micrograph (The deleted micrographs are marked with red circles). After removal both model 0 and 2 are executed on machine 0 at time step 0 (painted with blue square) which makes machine 2 idle at this time. The same problem occurs in time step 1. This uneven load on the number of computing tasks may results in longer overall computing time because not all machines are utilized at the same time.
\item How to distribute the training vertices from the removed micrographs to other micrographs? These vertices can not be directly deleted without training because this will result in a reduction in the number of training vertices and degrade GNN model accuracy.
\end{enumerate}
In one word, \textit{these questions can be described as determining how many and which time steps should be removed for each model}.
To this end, we propose the \techc{} algorithm. Three princeples are involved to answer the above questions. 

\begin{figure}
	\centering
	\includegraphics[width=3.2in]{et_our_remove.pdf}
	\caption{TT removal with \techc{} algorithm.}
	\label{fig:et_ours}
\end{figure}

Firstly, to ensure all models have the same total number of timesteps in each iteration training, the same number of micrographs are removed for each model. Because the exact execution time after removing one time step is unpredictable, we adopt a greedy approach. Specifically, starting from N, we attempt to iteratively decrease the numer of time step and measure the real end-to-end average epoch training time over three consecutive epochs after each reduction. This process continues until the average epoch training time increases or no longer decreases.

Secondly, to guarantee that different models are always trained on different machines at the same time step after removal, we adopt a column-wise approach for removing micrographs. Each time, we delete one column of the TT which represents a time step. After removal, the removed micrographs have to be reallocated to other time steps, which increases feature transmission between machines. To minimize the increased amount of feature transfer across machines,we prioritize removing the column with the smallest total number of vertices in the micrographs. In practice, we choose to remove the column with the smallest total number of root vertices, approximating the total number of vertices in the micrographs, which can reduce the sampling time when deciding which time step to be removed. 
For instance, in Figure~\ref{fig:et_ours}, the middle table illustrates the distribution of the number of training vertices in a mini-batch on each machine for each model. Assuming the mini-batch size of eight, thus the values in each row sum up to 8. To perform \techc{}, we calculate the total number of training vertices in each column, which is 9, 6, and 9, respectively. As a result, we opt to remove the middle column with the lowest total number of training vertices.

Lastly, to improve algorithm efficiency and ensure load balancing, we randomly and as evenly as possible allocate the training vertices from the removed micrographs to the preserved micrographs.

Putting all the above together, the details of \techc{} are shown in Algorithm~\ref{alg:reduce}.

\begin{algorithm}[t]
	\caption{\techC{} Algorithm.}
	\label{alg:reduce}
	\begin{algorithmic}[1]
		
		\Require
		$totalEpc$: total training epochs;
		
		$iTT$: the initial TT;
		
		$K$: calculate average time per K epochs;
		
		\State $curTT \gets iTT$
		\State $oldEpcTime = runKEpcGNN(curTT, K)$ \Comment{average epoch  time of K epochs with curTT}
		\State $curEpc \gets 0$ \Comment{current training epoch ID}
		\While {$curEpc <= totalEpc-K$} \Comment{training not finished}
		\If {$col\_counts(curTT) < 2$} 
		\State \Return $curTT$
		\EndIf
		
		\Statex\ // Trying to reduce time step.
		\State{$rootsD \gets redistribute\_roots(curTT)$} \Comment{redistribute root vertices according to curTT}
		\State{$colIndex \gets find\_fewest\_column(rootsD)$} \Comment{select column ID to remove}
		\State {$tmpCurTT \gets delete\_curTT\_cols(colIndex)$}
		
		\Statex\ // Training with tmpCurTT.
		\State {$newEpcTime \gets runGNN(tmpCurTT, K)$}
		\State {$curEpc \gets curEpc + K$}
		\If {$newEpcTime < oldEpcTime$}
		\State {$curTT \gets tmpCurTT$} \Comment{update curTT}
		\State {$oldEpcTime \gets newEpcTime$}
		\Else
		\State \Return $curTT$
		\EndIf
		\EndWhile
	\end{algorithmic}
	%     \vspace{-0.05in}
\end{algorithm}

==> tex/exp-overhead.tex <==
%\subsection{Overhead Analysis}
%\label{exp:overhead}
